LLMs Meet Library Evolution: Evaluating Deprecated API Usage in LLM-based Code Completion

Large language models (LLMs), pre-trained or fine-tuned on large code corpora, have shown effectiveness in generating code completions. However, in LLM-based code completion, LLMs may struggle to use correct and up-to-date Application Programming Interfaces (APIs) due to the rapid and continuous evolution of libraries. While existing studies have highlighted issues with predicting incorrect APIs, the specific problem of deprecated API usage in LLM-based code completion has not been thoroughly investigated. To address this gap, we conducted the first evaluation study on deprecated API usage in LLM-based code completion. This study involved seven advanced LLMs, 145 API mappings from eight popular Python libraries, and 28,125 completion prompts. The study results reveal the status quo (i.e., API usage plausibility and deprecated usage rate) of deprecated API and replacing API usage in LLM-based code completion from the perspectives of model, prompt, and library, and indicate the root causes behind. Based on these findings, we propose two lightweight fixing approaches, REPLACEAPI and INSERTPROMPT, which can serve as baseline approaches for future research on mitigating deprecated API usage in LLM-based completion. Additionally, we provide implications for future research on integrating library evolution with LLM-driven software development.

==> src/results-bak.tex <==
\section{Study Results}
In this section, we present the experimental results and key findings for answering the aforementioned research questions.

% \todo{Maybe we should reorganize the RQs. Should be the cause analysis merged into result presentation?}

\subsection{RQ1: Functional Correctness in LLM-based Code Completion}\label{sec:rq1}
The distribution of \good and \bad completions shown in Figure~\ref{fig:rq1-overall}, along with the low \fcr metric presented in Table~\ref{tab:rq1-overall}, highlights that all the LLMs encountered challenges in accurately predicting functionally correct APIs for prompts from both $\mathcal{B}$ and $\mathcal{F}$. 

\begin{figure}
    \includegraphics[width=\columnwidth]{img/rq1-overall.pdf}
    \caption{Distribution of \good, \bad, and \irrelevant completions by LLMs for prompts from $\mathcal{B}$ and $\mathcal{F}$.}
    \label{fig:rq1-overall}
\end{figure}

% \begin{table}
%     \caption{FCR and DUR metrics for $\mathcal{B}$, $\mathcal{F}$, and overall dataset (\ie All = $\mathcal{B} \cup \mathcal{F}$).}
%     \label{tab:rq1-overall}
%     \centering
%     \renewcommand{\arraystretch}{1.2}
%     \setlength{\tabcolsep}{4pt}
%     \begin{tabularx}{0.95\columnwidth}{l|cYYYcYYY}
%     \Xhline{2\arrayrulewidth}
%     \multirow{2}{*}{\textbf{Model}} & & \multicolumn{3}{c}{\textbf{FCR (\%)}} & & \multicolumn{3}{c}{\textbf{DUR (\%)}} \\
%     \cline{3-5}\cline{7-9}
%     & & $\mathcal{B}$ & $\mathcal{F}$ & All & & $\mathcal{B}$ & $\mathcal{F}$ & All \\
%     \Xhline{1.5\arrayrulewidth}
%     CodeGen-350m & & \heatmapcell{8.6} & \heatmapcell{14.2} & \heatmapcell{12.3} & & \heatmapcell{77.7} & \heatmapcell{9.0} & \heatmapcell{24.9} \\
%     CodeGen-2b & & \heatmapcell{19.0} & \heatmapcell{25.2} & \heatmapcell{23.1} & & \heatmapcell{89.6} & \heatmapcell{11.3} & \heatmapcell{32.6} \\
%     CodeGen-6b & & \heatmapcell{26.1} & \heatmapcell{30.9} & \heatmapcell{29.3} & & \heatmapcell{90.0} & \heatmapcell{11.1} & \heatmapcell{34.2} \\
%     DeepSeek-1.3b & & \heatmapcell{10.2} & \heatmapcell{13.4} & \heatmapcell{12.3} & & \heatmapcell{69.7} & \heatmapcell{11.6} & \heatmapcell{27.2} \\
%     StarCoder-3b & & \heatmapcell{8.8} & \heatmapcell{10.9} & \heatmapcell{10.2} & & \heatmapcell{79.4} & \heatmapcell{17.0} & \heatmapcell{34.4} \\
%     CodeLlama-7b & & \heatmapcell{27.6} & \heatmapcell{32.1} & \heatmapcell{30.6} & & \heatmapcell{86.9} & \heatmapcell{12.1} & \heatmapcell{34.2} \\
%     GPT-3.5 & & \heatmapcell{13.5} & \heatmapcell{16.0} & \heatmapcell{15.2} & & \heatmapcell{85.7} & \heatmapcell{17.8} & \heatmapcell{37.4} \\
%     \Xhline{2\arrayrulewidth}
%     \end{tabularx}
% \end{table}


\begin{table}
    \caption{FCR for $\mathcal{B}$, $\mathcal{F}$, and overall dataset (\ie All = $\mathcal{B} \cup \mathcal{F}$).}
    \label{tab:rq1-overall}
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{4pt}
    \begin{tabularx}{0.8\columnwidth}{l|cYYY}
    \Xhline{2\arrayrulewidth}
    \multirow{2}{*}{\textbf{Model}} & & \multicolumn{3}{c}{\textbf{FCR (\%)}} \\
    \cline{3-5}
    & & $\mathcal{B}$ & $\mathcal{F}$ & All\\
    \Xhline{1.5\arrayrulewidth}
    CodeGen-350m & & \heatmapcell{8.6} & \heatmapcell{14.2} & \heatmapcell{12.3} \\
    CodeGen-2b & & \heatmapcell{19.0} & \heatmapcell{25.2} & \heatmapcell{23.1} \\
    CodeGen-6b & & \heatmapcell{26.1} & \heatmapcell{30.9} & \heatmapcell{29.3} \\
    DeepSeek-1.3b & & \heatmapcell{10.2} & \heatmapcell{13.4} & \heatmapcell{12.3} \\
    StarCoder-3b & & \heatmapcell{8.8} & \heatmapcell{10.9} & \heatmapcell{10.2} \\
    CodeLlama-7b & & \heatmapcell{27.6} & \heatmapcell{32.1} & \heatmapcell{30.6} \\
    GPT-3.5 & & \heatmapcell{13.5} & \heatmapcell{16.0} & \heatmapcell{15.2} \\
    \Xhline{2\arrayrulewidth}
    \end{tabularx}
\end{table}


\textbf{Model Perspective.}
The \fcr of the LLMs for overall dataset (\ie All $=\mathcal{B}\cup\mathcal{F}$) ranges from 10\% to 30\%, indicating that a majority of predictions were \irrelevant. Among the LLMs, CodeLlama-7b achieved the highest \fcr (30.6\%), while StarCoder2-3b had the lowest overall \fcr (10.2\%). This may be attributed to the fact that StarCoder2 was not specifically fine-tuned on additional Python corpora, unlike other LLMs such as CodeLlama and CodeGen. 
Comparing the three versions of CodeGen suggests that the capacity of LLMs to predict functionally correct APIs increased with model size (\ie 12.3\%, 23.1\%, and 29.3\% for CodeGen-350m, -2b, and -6b, respectively), given the model architecture and training data remain consistent. However, it's noteworthy that the largest LLM, GPT-3.5, did not achieve a high \fcr (15.2\%), possibly due to the instruction used not being finely tuned with advanced prompt engineering techniques such as chain-of-thought (COT)~\cite{COT} and in-context learning (ICL)~\cite{ICL}.


\finding{
All the evaluated LLMs faced challenges in accurately predicting functionally correct APIs, with \fcr ranging from 10\% to 30\%. Effectiveness of the LLMs in Python code completion generally improved with model size and language-specific fine-tuning.
}

\textbf{Prompt Perspective.}
Between the prompts from the two different datasets, $\mathcal{B}$ and $\mathcal{F}$, there are differences in \fcr for all LLMs, with relative differences (\ie $(\fcr_{\mathcal{F}} - \fcr_{\mathcal{B}}) / \fcr_{\mathcal{B}}$) ranging from 16\% to 65\%. This disparity may be attributed to the imbalance in the number of \buggy and \fixed functions in the LLMs' training corpora~\cite{Imbalance1,Imbalance2}. Indirect evidence for this is that, in this study, the \fixed functions collected from open-source code repositories were about twice as many as the \buggy functions (\ie 19,103 \emph{vs.} 9,022), even though there was no collection preference. Given that LLMs were often trained on open-source code repositories, we can conclude that the LLMs were trained on more \fixed functions than \buggy functions, leading to better \fcr for the $\mathcal{F}$ dataset. Additionally, larger LLMs showcased smaller \fcr differences (\eg 16\% for CodeLlama-7b and 65\% for CodeGen-350m), possibly due to their better generalizability.

\finding{
All the LLMs showcased difference in \fcr between the two datasets $\mathcal{B}$ and $\mathcal{F}$. This difference is possibly attributed to the different distribution of \buggy and \fixed functions in the training corpora of LLMs.
}

\textbf{Library Perspective.}
We also conducted a detailed analysis to examine the LLMs' effectiveness in predicting functionally correct APIs across different libraries, focusing on how \fcr vary with different libraries. The results are illustrated in the scatter plots depicted in Figure~\ref{fig:rq1-library-fcr}, where each data point signifies the \fcr of an LLM for a specific library. Across the 8 libraries, most LLMs exhibited relatively low functional correctness for both $\mathcal{B}$ and $\mathcal{F}$, with \fcr below 30\%. Notable exceptions were Pandas and TensorFlow, where CodeLlama-7b, CodeGen-6b, and CodeGen-2b (represented by symbols ``\mystar'',  ``\trialeft'', and ``\triaup'', respectively) achieved better \fcr (around or greater than 40\%). This aligns with the results presented in Model Perspective, where CodeLlama-7b, CodeGen-6b, and CodeGen-2b achieved the best results for the overall dataset. On the other hand, among the libraries, completion prompts from SciPy and seaborn posed the most difficulty for LLMs in predicting functionally correct APIs, with \fcr consistently below 15\%. 

\todo{The following analysis may be more suitable for RQ2...}
After analyzing the completion prompts and LLMs' predictions, we found that the \fcr differences between these libraries were primarily due to the characteristics of the API usage context. 
More specifically, the usage contexts of certain APIs followed common patterns and were surrounded by related APIs, allowing advanced LLMs like CodeLlama-7b to infer the desired API functionality based on the completion prompt. For example, many utility APIs in TensorFlow, such as the deprecated \inlinecode{tensorflow.compat.v1.initialize\_all\_variables} and its replacement \inlinecode{tensorflow.compat.v1.global\_variables\_initializer}, were often used in recognizable patterns that were easier for LLMs to predict. Conversely, some APIs were used more flexibly in diverse contexts and lacked obvious combinations with other APIs, leading to low \fcr for LLMs in predicting such APIs. For instance, many APIs in SciPy, like the deprecated \inlinecode{scipy.misc.comb} and its replacement \inlinecode{scipy.special.comb}, can be used in diverse contexts to produce combinations for a data sequence. Since the data sequence can originate from numerous sources and be structured in various ways (\eg Numpy array and Pandas Series), it is challenging for LLMs to predict these APIs based on the completion prompt without additional hints. 

\begin{figure}
    \includegraphics[width=\columnwidth]{img/rq1-library-fcr.pdf}
    \caption{\fcr of LLMs across libraries.}
    \label{fig:rq1-library-fcr}
\end{figure}

\finding{
Most LLMs exhibited relatively low functional correctness across the 8 libraries, with \fcr below 30\%. The \fcr differences between these libraries were primarily due to the different characteristics of API usage contexts. 
}




\subsection{RQ2: Deprecated Usage in Functionally Correct Completions}
The distribution of \good and \bad completions shown in Figure~\ref{fig:rq1-overall}, along with the \dur metric presented in Table~\ref{tab:rq1-overall}, indicates that all LLMs faced issues with using deprecated API usage.


\begin{table}
    \caption{FCR and DUR metrics for $\mathcal{B}$, $\mathcal{F}$, and overall dataset (\ie All = $\mathcal{B} \cup \mathcal{F}$).}
    \label{tab:rq1-overall}
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{4pt}
    \begin{tabularx}{0.8\columnwidth}{l|cYYY}
    \Xhline{2\arrayrulewidth}
    \multirow{2}{*}{\textbf{Model}} & & \multicolumn{3}{c}{\textbf{DUR (\%)}} \\
    \cline{3-5}
    & & $\mathcal{B}$ & $\mathcal{F}$ & All \\
    \Xhline{1.5\arrayrulewidth}
    CodeGen-350m & & \heatmapcell{77.7} & \heatmapcell{9.0} & \heatmapcell{24.9} \\
    CodeGen-2b & & \heatmapcell{89.6} & \heatmapcell{11.3} & \heatmapcell{32.6} \\
    CodeGen-6b & & \heatmapcell{90.0} & \heatmapcell{11.1} & \heatmapcell{34.2} \\
    DeepSeek-1.3b & & \heatmapcell{69.7} & \heatmapcell{11.6} & \heatmapcell{27.2} \\
    StarCoder-3b & & \heatmapcell{79.4} & \heatmapcell{17.0} & \heatmapcell{34.4} \\
    CodeLlama-7b & & \heatmapcell{86.9} & \heatmapcell{12.1} & \heatmapcell{34.2} \\
    GPT-3.5 & & \heatmapcell{85.7} & \heatmapcell{17.8} & \heatmapcell{37.4} \\
    \Xhline{2\arrayrulewidth}
    \end{tabularx}
\end{table}

\textbf{Model Perspective.}
The \dur of the LLMs for the overall dataset (\ie All $=\mathcal{B}\cup\mathcal{F}$) ranges from 25\% to 38\%, with larger models (\eg CodeGen-6b, CodeLlama-7b, and GPT-3.5) generally predicting more usages of deprecated APIs. \todo{Why?...} %This trend may be attributed to the increased complexity and broader training data of larger models, which could include more deprecated API examples.
Considering the differences among the LLMs, CodeLlama-7b and CodeGen-6b demonstrated the best balance between \fcr and \dur. They achieved significant improvements in \fcr compared to other LLMs, with a comparable \dur of 34.2\%. Conversely, StarCoder2-3b and GPT-3.5 exhibited higher \dur (\ie 34.4\% and 37.4\%) despite having much lower \fcr. These results indicate that the preference of LLMs for using deprecated or replacement APIs is not closely related to their capacity for predicting functionally correct completions. \todo{Maybe related to training data?}

\finding{
All the evaluated LLMs faced issues with deprecated API usage, with \dur ranging from 25\% to 38\%, and larger models exhibiting higher \dur. Among the LLMs, CodeLlama-7b and CodeGen-6b demonstrated the best balance between \fcr and \dur.
}

\textbf{Prompt Perspective.}
When considering $\mathcal{B}$ and $\mathcal{F}$ separately, all LLMs consistently demonstrated extremely high deprecated API usage rates for $\mathcal{B}$ (70\%-90\% \dur) and relatively low rates for $\mathcal{F}$ (9\%-18\% \dur). This significant difference is also evident in the distribution of \good and \bad completions shown in Figure~\ref{fig:rq1-overall}. It may be attributed to certain contextual characteristics of the prompts from $\mathcal{B}$ that led the LLMs to predict deprecated APIs, while the differing characteristics of prompts from $\mathcal{F}$ led to the prediction of replacement APIs instead. In fact, for functionally correct completions, the rate of \emph{reference} API usage (\ie the API used in the original function) equals \fcr for $\mathcal{B}$, while it is $(1 - \fcr)$ for $\mathcal{F}$. 
Considering this rate, there is no noticeable difference between $\mathcal{B}$ and $\mathcal{F}$ (\ie around 70\%-90\% for both). This suggests that LLMs predicted the reference APIs for most prompts from both datasets, aided by their differing code contextual characteristics. Despite accounting for the contextual characteristics, the 9\%-18\% \dur for $\mathcal{F}$ indicates that LLMs still predicted the usage of deprecated APIs, even for the prompts from \fixed functions.


\finding{
All LLMs consistently exhibited a significant difference in \dur between the two datasets, $\mathcal{B}$ and $\mathcal{F}$, with extremely high deprecated API usage rates for $\mathcal{B}$ (70\%-90\% \dur) and relatively low rates for $\mathcal{F}$ (9\%-18\% \dur). This large disparity is likely due to the differing contextual characteristics between $\mathcal{B}$ and $\mathcal{F}$.
}


\textbf{Library Perspective.}
We performed an in-depth analysis to evaluate the use of deprecated APIs by the LLMs across different libraries, specifically examining how \dur varies among the libraries. The results are presented in the scatter plots shown in Figure~\ref{fig:rq1-library-dur}, where each data point represents the \dur of a particular LLM for a specific library. The results reveal significant differences in the usage of deprecated APIs across the libraries, with \dur ranging from approximately 0\% to 100\%. Specifically, LLMs generally showed low \dur (around or below 20\%) for Numpy, scikit-learn, and TensorFlow. In contrast, LLMs exhibited consistently high \dur for SciPy (approximately 30\%-50\%) and PyTorch (approximately 50\%-70\%), and unstable \dur for Pandas (approximately 30\%-80\%) and Transformers (approximately 40\%-100\%). These significant differences across libraries were primarily attributed to the varying characteristics of evolution and API deprecations of different libraries, which caused LLMs to behave differently in utilizing deprecated APIs for different libraries.




\begin{figure}
    \includegraphics[width=\columnwidth]{img/rq1-library-dur.pdf}
    \caption{\dur of LLMs across libraries.}
    \label{fig:rq1-library-dur}
\end{figure}

\finding{
LLMs showed significant differences in the usage of deprecated APIs across various libraries, with \dur ranging from approximately 0\% to 100\%. These variations in \dur were primarily due to the differing characteristics of library evolution and API deprecations.
}




\subsection{RQ3: Root Causes of Deprecated API Usages}
Since the use of deprecated APIs can introduce unreliable factors such as software vulnerabilities~\cite{sigsoft/Wang0LC20}, it is essential to conduct an in-depth analysis to identify the root causes of deprecated API usage in LLM-based code completion. In this analysis, we also present the results from three perspectives: Model, Prompt, and Library.

\textbf{Model Perspective.}
From the model perspective, the causes of deprecated API usage can be divided into two main points:
\begin{itemize}
    \item \textbf{Model Training:} The LLMs were trained on large-scale code corpora, primarily collected from code repositories. As libraries evolved, both deprecated APIs and their replacements were used in software development, leading to training corpora containing instances of deprecated API usage. For instance, in this study, we collected 9,022 functions from open-source code corpora that used deprecated APIs. When trained on such data, LLMs might ``memorize'' these deprecated APIs and their usage contexts as part of the learned knowledge~\cite{LLM-KB,LLM-KB-Revisiting}.
    \item \textbf{Model Inference:}  During the inference stage, LLMs generated completions by predicting token probabilities based on their learned \emph{prior} knowledge (\eg the memorized API usage contexts) and applying token selection strategies (\eg greedy search or beam search). Given certain contexts, LLMs were likely to predict deprecated API usages due to the high token probabilities, without considering any \emph{posterior} knowledge about API deprecations.
\end{itemize}

\finding{
There are two primary reasons why LLMs predict deprecated APIs: the presence of deprecated API usages in the training corpora during the training stage, and the absence of posterior knowledge about API deprecations during the inference stage.
}

\textbf{Prompt Perspective.}
The contextual characteristics of the input completion prompts can significantly influence LLMs' use of deprecated APIs. Since the completions are generated based on the input prompts, specific contexts can lead LLMs to use deprecated APIs. As presented in RQ2, the LLMs showed significantly different \dur for prompts from $\mathcal{B}$ and $\mathcal{F}$, respectively. Upon comparing the prompts from the two datasets, we found that prompts from $\mathcal{B}$ often contained specific characteristics related to API usage contexts, such as different objects, control flows, and data flows, which prompted the LLMs to use deprecated APIs instead of their replacements. For example, \todo{examples... Maybe need a statistics to support the statement.}


\textbf{Library Perspective.}
The characteristics of API deprecations during library evolution also significantly impacted the use of deprecated APIs in LLM-based code completions. Some APIs were deprecated due to simple package refactoring, leading to similar usage patterns for the deprecated APIs and their replacements. For example, in the version 1.9.0 release of PyTorch, many APIs for tensor linear algebra were moved from the \inlinecode{torch} package to the \inlinecode{torch.linalg} package without changes to the API parameters or usage patterns (\eg \inlinecode{torch.lstsq} $\to$ \inlinecode{torch.linalg.lstsq}). In such cases, LLMs found it more difficult to distinguish between deprecated APIs and their replacements, resulting in more frequent use of deprecated APIs in the predicted completions.

 

==> src/threats.tex <==
\section{Threats to Validity}
\textbf{Internal Threats.}
The primary threat to the internal validity of our study is the soundness of the static analysis used for function location and result annotation. Given that Python is a dynamic programming language, the lightweight object type resolution method we employed may have missed some function calls of deprecated and replacing APIs during the matching process. In the future, we aim to address this issue by implementing advanced type inference techniques. Additionally, our study currently focuses on function-level API deprecation, overlooking parameter-level deprecations. Future research should investigate a broader range of deprecated API categories to provide a more comprehensive analysis.

\textbf{External Threats.}
A primary threat to the external validity of our study lies in the choice of Python libraries and the evaluated LLMs. To mitigate this threat, we reused libraries examined in previous studies and introduced three popular deep learning libraries to ensure diversity and timeliness. For the LLMs, we selected models covering various architectures, model sizes, training corpora, and training strategies to ensure the generalizability of our findings. Another external threat is that the study was conducted solely on the Python language, which may limit the applicability of our findings to other languages such as Java and C\#. In the future, we plan to explore the impact of library evolution on LLM-based code completion across a broader range of programming languages.
